A semiparametric Bayesian approach to epidemics, with application to the spread of the coronavirus MERS in South Korea in 2015

We consider incomplete observations of stochastic processes governing the spread of infectious diseases through finite populations by way of contact. We propose a flexible semiparametric modeling framework with at least three advantages. First, it enables researchers to study the structure of a population contact network and its impact on the spread of infectious diseases. Second, it can accommodate short- and long-tailed degree distributions and detect potential superspreaders, who represent an important public health concern. Third, it addresses the important issue of incomplete data. Starting from first principles, we show when the incomplete-data generating process is ignorable for the purpose of Bayesian inference for the parameters of the population model. We demonstrate the semiparametric modeling framework by simulations and an application to the partially observed MERS epidemic in South Korea in 2015. We conclude with an extended discussion of open questions and directions for future research.

==> combinations.tex <==
or some combinations of the above.


==> contents.tex <==
\bi
\item[] Section 1 Motivation
\bi
\item[] Section 1.1 Advantages of network-based approaches to epidemics
\item[] Section 1.2 Shortcomings of existing network-based approaches
\item[] Section 1.3 Proposed network-based approach 
\item[] Section 1.4 Goal: superpopulation inference for finite populations
\item[] Section 1.5 Structure of the paper
\ei
\item[] Section 2 A network-based stochastic model of epidemics
\bi
\item[] Section 2.1 Data-generating process
\item[] Section 2.2 Parametric population models
\ei
\item[] Section 3 Shortcomings of parametric population models
\item[] Section 4 Semiparametric population model
\bi
\item[] Section 4.1 Detecting potential superspreaders
\item[] Section 4.2 Short- and long-tailed degree distributions
\ei
\item[] Section 5 Incomplete data
\bi
\item[] Section 5.1 Possible reasons for incomplete data
\item[] Section 5.2 Importance of collecting network data
\ei
\item[] Section 6 Bayesian inference
\bi
\item[] Section 6.1 Complete- and incomplete-data generating process
\item[] Section 6.2 Bayesian inference based on incomplete data
\item[] Section 6.3 Truncated Dirichlet process priors
\item[] Section 6.4 Bayesian Markov chain Monte Carlo algorithm
\item[] Section 6.5 Addressing the label-switching problem
\ei
\item[] Section 7 Simulation results
\bi
\item[] Section 7.1 Simulation results quantifying the error of estimation
\item[] Section 7.2 Simulation results quantifying the effect of network sampling
\ei
\item[] Section 8 Partially observed MERS epidemic in South Korea
\bi
\item[] Section 8.1 Data
\item[] Section 8.2 Model
\item[] Section 8.3 Computing
\item[] Section 8.4 Results
\ei
\item[] Section 9 Open questions and directions for future research
\bi
\item[] Section 9.1 What is the population of interest?
\item[] Section 9.2 Incomplete data
\item[] Section 9.3 Computational challenges arising from incomplete data
\item[] Section 9.4 Non-ignorable incomplete-data generating processes
\item[] Section 9.5 Population models capturing additional network features
\item[] Section 9.6 Time-evolving population contact networks
\ei
\ei


==> more.data.tex <==
It is worth noting that,
in addition to the assessments of doctors,
the observed infectious and removal times help inform who infected whom.
To see that,
note that we know who is infectious in a given time interval,
because we observe the infectious and removal times of infected population members.
Suppose that population member $1$ turns infectious on day 1 and recovers by day 14 and population member $2$ turns infectious on day 7,
while all other population members are non-infectious during the first two weeks of the epidemic.
Then population member $1$ must have infected population member $2$ during the first week of the epidemic.
In other words,
the observed infectious and removal times can reduce the posterior uncertainty about who infected whom,
by narrowing down the possible sources of infections.


==> mse.plot.tex <==
Simulation results: MSE of the posterior median and mean of the parameters $\beta$, $\gamma_1$, $\gamma_2$, and $\gamma_3$ plotted against the sample size $n = 0$,\, $25$,\, $50$,\, $75$,\, $100$,\, $125$,\, $150$,\, $187$.\break
If $n=0$,
no contacts are observed,
otherwise a subset of contacts is observed.


==> mse.tex <==
1,000 egocentric samples of size $n = 25$, $50$, $75$, $100$, $125$, $150$, $187$ are generated from the population of size $N = 187$.
For each sample, 
we estimated the model.
In addition,
we estimated the model without observations of contacts,
that is,
when $n=0$.
The MSE of the posterior median and mean of the rate of infection $\beta$ and the degree parameters $\gamma_1, \gamma_2, \gamma_3$ are shown in Figure \ref{mse.plot} when $n = 0$, $25$, $50$, $75$, $100$, $125$, $150$, $187$.
By construction of the model,
estimators of the epidemiological parameters $\eta_{E,1}$, $\eta_{E,2}$, $\eta_{I,1}$, $\eta_{I,2}$ are not expected to be sensitive to $n$---which determines how much information is available about the network parameters---and the MSE of the posterior median and mean of $\eta_{E,1}$, $\eta_{E,2}$, $\eta_{I,1}$, $\eta_{I,2}$ is indeed not sensitive to $n$ (not shown).
Figure \ref{mse.plot} demonstrates that samples of contacts reduce the MSE of posterior median and mean of $\beta$, $\gamma_1, \gamma_2, \gamma_3$:           
The MSE turns out to be highest when $n = 0$,
%A sample of size $n=25$ results in a large reduction in MSE,
%and increasing $n$ tends to decrease the MSE.
and rapidly decreases as $n$ increases.
These observations suggest that in practice samples of contacts---or functions of contacts, 
such as degrees---should be collected,
reducing posterior uncertainty.


==> sims.tex <==
By construction of the model,
estimators of the epidemiological parameters $\eta_{E,1}$, $\eta_{E,2}$, $\eta_{I,1}$, and $\eta_{I,2}$ are not expected to be sensitive to $n$---which determines how much information is available about the network parameters---and the MSE of the posterior median and mean of $\eta_{E,1}$, $\eta_{E,2}$, $\eta_{I,1}$, and $\eta_{I,2}$ are indeed not sensitive to $n$ (not shown).
But Figure 4 demonstrates that samples of contacts do reduce the MSE of the posterior median and mean of $\beta$, $\gamma_1$, $\gamma_2$, and $\gamma_3$:
The MSE turns out to be highest when $n = 0$,
%A sample of size $n=25$ results in a large reduction in MSE,
%and increasing $n$ tends to decrease the MSE.
and rapidly decreases as $n$ increases.
These observations underscore the importance of collecting data on contacts or functions of contacts,
such as degrees.


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
\tikzstyle{inf} = [latent,fill=red]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


